Light curves of transneptunian objects from the K2 mission of the Kepler Space Telescope

The K2 mission of the Kepler Space Telescope allowed the observations of light curves of small solar system bodies throughout the whole Solar system. In this paper we present the results of a collection of K2 transneptunian object observations, between Campaigns C03 (November 2014 -- February 2015) to C19 (August -- September, 2018), which includes 66 targets. Due to the faintness of our targets the detectability rate of a light curve period is $\sim$56%, notably lower than in the case of other small body populations, like Hildas or Jovian trojans. We managed to obtain light curve periods with an acceptable confidence for 37 targets; the majority of these cases are new identifications. We were able to give light curve amplitude upper limits for the other 29 targets. Several of the newly detected light curve periods are longer than $\sim$24 h, in many cases close to $\sim$80 h, i.e., these targets are slow rotators. This relative abundance of slowly rotating objects is similar to that observed among Hildas, Jovian trojans and Centaurs in the K2 mission, and also among main belt asteroids measured with the TESS Space Telescope. Transneptunian objects show notably higher light curve amplitudes at large (D $\gtrsim$ 300 km) sizes than that found among large main belt asteroids, in contrast to the general expectation that due to their lower compressive strength they reach hydrostatic equlibrium at smaller sizes than their inner solar system counterparts.

==> aei.tex <==
\startlongtable
\begin{deluxetable*}{cccccc}
\tabletypesize{\scriptsize}
\tablecaption{Summary table of the main orbital characteristics and dynamical classification of our targets. The columns are: (1) name and/or provisional designation; (2) V-band absolute magnitude (mag); (3) semi-major axis (au);
(4) eccentricity; (5) inclination (deg); (6) dynamical class or mean-motion resonance with Neptune. Cold and hot classicals are separated by the inclination i\,=\,4\fdg5 \citep[see e.g.][]{Gladman2008}. } %\label{tab:largetable}
\tablehead{\colhead{Name}  & \colhead{H$_{V}$}  & \colhead{a}  &  \colhead{e}  &  \colhead{i}  
&  \colhead{Dynamical group}
}
\colnumbers
\startdata
\sn & 5.68 & 37.8239563 & 0.0399826 & 4.61245 & hot classical\\ 
\de & 4.94 & 55.5040117 & 0.4168371 & 7.62938 & 2:5 resonance\\
\cm & 6.68 & 42.1255750 & 0.0640919 & 3.75516 & cold classical\\  
\ok & 6.0 & 46.5813354 & 0.1403453 & 4.88465 & hot classical\\ 
\hz & 6.6 & 43.0180466 & 0.0323816 & 2.93273 & cold classical\\ 
\kn & 6.6 & 44.0637410 & 0.0956953 & 2.64496 & cold classical\\
\qb & 6.8 & 42.7192221 & 0.0995969 & 1.79485 & cold classical\\
\qj & 6.2 & 44.1753883 & 0.0365290 & 2.15477 & cold classical\\
\qt & 6.2 & 37.0258514 & 0.0220311 & 1.84662 & inner classical\\
\qx & 6.3 & 44.2115741 & 0.0270365 & 0.90745 & cold classical\\
\xd & 5.8 & 39.2882985 & 0.1118632 & 18.14109 & plutino\\
\xp & 7.77 & 42.0465415 & 0.2142201 & 2.61611 & 3:5 resonance\\
\xu & 6.68 & 43.2829795 & 0.0780917 & 6.52230 & hot classical\\
\yh & 5.58 & 42.1828001 & 0.1369339 & 11.09996 & 3:5 resonance\\
\cy & 6.16 & 53.7570643 & 0.3432009 & 15.76009 & 5:12 resonance\\
\gj & 5.4 & 44.5446573 & 0.1073526 & 11.57225 & hot classical\\  
%\gv & 6.4 & 44.1114402 & 0.0934619 & 2.18150 & cold classical \\
\vs & 6.3 & 44.8124374 & 0.1201659 & 3.00131 & cold classical\\
\vt & 5.7 & 42.2145036 & 0.0356054 & 1.16426 & cold classical\\
\vu & 5.9 & 38.9541796 & 0.2103117 & 1.37856 & plutino\\
\fe & 6.37 & 48.4332947 & 0.2592514 & 3.38301 & 1:2 resonance\\
\gh & 6.0 & 44.4898956 & 0.0844735 & 1.10267 & cold classical\\
\qa & 6.9 & 38.2803717 & 0.0583336 & 3.42715 & inner classical\\
\ys & 6.8 & 43.4354691 & 0.0266317 & 3.73349 & cold classical\\
\fc & 7.41 & 35.0390366 & 0.0839447 & 2.37160 & 4:5 resonance\\
\qw  & 5.0 & 43.6941429 & 0.0734856 & 10.36787 & hot classical\\
\xr & 4.3 & 57.2561486 & 0.1073786 & 46.79343 & scattered disk\\
\tf & 6.3 & 79.8663748 & 0.5072393 & 23.23663 & scattered disk\\
\tv & 6.9 & 47.3800039 & 0.2722973 & 9.78559 & 1:2 resonance\\
\eo & 6.21 & 45.8983194 & 0.0739658 & 3.41227 & cold classical\\
\ez & 7.13 & 39.6766516 & 0.1557282 & 1.77550 & plutino\\
\tb & 4.55 & 75.9529877 & 0.3917797 & 26.49004 & scattered disk\\
\rs & 5.18 & 47.7306105 & 0.2003342 & 10.02598 & 1:2 resonance\\
%\jj & 4.5 & 48.4335712 & 0.1667240 & 12.02150 & other TNO\\
%\orten & 1.92 & 67.3782754 & 0.5029745 & 30.73943 & 3:10 resonance\\  
\cs & 6.27 & 42.2933803 & 0.1579361 & 15.94423 & 3:5 resonance\\
\yg & 6.2 & 55.2226347 & 0.4040541 & 5.16230 & 2:5 resonance \\
\ep & 5.54 & 47.8794282 & 0.3094197  & 18.86373 & 1:2 resonance\\
\et & 5.26 & 62.5104891 & 0.3659258 & 30.58345 & scattered disk\\
\fcten  & 5.88 & 39.0790779 & 0.0535418 & 39.73235 & plutino\\
\jf & 5.43 & 41.6753240 & 0.1307786 & 27.64613 & hot classical  \\
\dw & 6.06 & 41.2840227 & 0.0379671 & 18.99296 & hot classical\\
\apthirteen & 5.67 & 57.5543033 & 0.3668924 & 3.33318 & 3:8 resonance\\
\at & 4.9 & 61.6173083 & 0.4217387 & 28.12567 & scattered disk\\
\fa & 6.2 & 44.4091197 & 0.0426125 & 1.53768 & cold classical\\
\jv & 6.35 & 42.9996513 & 0.0424042 & 3.21441 & cold classical\\
\am & 5.2 & 47.0230084 & 0.1423797 & 7.18355 & hot classical\\
\df & 5.56 & 42.8307595 & 0.0456454 & 23.68086 & hot classical\\
\djfourteen & 6.61 & 38.1807753 & 0.0232355 & 6.93181 & 4:13 resonance\\
\ezfourteen & 3.92 & 52.5242987 & 0.2263985 & 10.25719 & scattered disk\\
\gdfourteen & 6.71 & 90.1672371 & 0.6157590 & 4.74239 & scattered disk\\
\gefourteen & 6.56 & 56.0228149 & 0.4158196 & 0.80808 & 2:5 resonance\\ 
\gjfourteen & 7.5 & 39.8224386 & 0.2801272 & 17.22611 & plutino\\
\hf & 5.9 & 61.7601933 & 0.4255242 & 9.71007 & scattered disk\\
\jq & 7.38 & 39.7549394 & 0.2233159 & 7.97258 & plutino\\
\ls & 6.2 & 43.6029549 & 0.0681892 & 3.82390 & cold classical\\
\wanine & 6.0 & 44.0261031 & 0.0531885 & 3.00216 & cold classical\\
\waten & 5.9 & 45.4170544 & 0.0367855  & 2.15623 & cold classical\\
\wj & 6.71 & 68.4462110 & 0.4912992 & 24.36183 & scattered disk\\
\wo & 6.3 & 43.9992014  & 0.0923767  & 3.75719 & cold classical\\
\ws & 5.55 & 54.9409609 & 0.3708612 & 8.90970 & 2:5 resonance\\
\ye & 5.53 & 59.1067258 & 0.3757100 & 26.91854 & scattered disk\\
\yj & 6.84 & 39.3040558 & 0.1951859 & 7.28212 & plutino\\
\bbfifteen & 6.7 & 63.1405090  & 0.4398171 & 27.62710 & scattered disk\\
\bc & 6.7 & 55.2299967  & 0.4166677 & 1.72294 & 2:5 resonance\\
\bz & 4.81 & 47.2750427 & 0.1850024 & 11.35989 & other TNO\\
\da & 7.47  & 72.9126980 & 0.5110819 & 27.66698 & scattered disk\\
Borasisi & 5.9 & 43.8343021 & 0.0906165 & 0.56342 & cold classical\\
Praamzius & 5.75 & 42.5834453 & 0.0104114 & 1.09950 & cold classical\\ \hline
%Pluto  & -0.45 & 39.8461080 & 0.2537532 & 17.10337 & \\
%Quaoar & 2.51    & 43.6913200 & 0.0395534 & 7.98813 & cubewano\\ \hline
\enddata
\end{deluxetable*}
%\endlongtable
\normalsize

%cubewano 4.5 inkclinacio alatt cold, felette hot

==> aei_m11r.tex <==
\startlongtable
\begin{deluxetable*}{lccccc|ccc}
\tabletypesize{\scriptsize}
\tablecaption{Summary table of the main orbital characteristics and dynamical classification of our targets. 
The columns are: (1) name and/or provisional designation; (2) V-band absolute magnitude (mag); (3) semi-major axis (au);
(4) eccentricity; (5) inclination (deg); (6) dynamical class or mean-motion resonance with Neptune. 
Cold and hot classicals are separated by the inclination i\,=\,4\fdg5 \citep[see e.g.][]{Gladman2008}; 
(7) phase-angle-uncorrected mean absolute brightness (Kepler\,$\approx$\,R-band, mag); (8) mean phase angle (deg);
(9) phase-angle-corrected mean absolute brightness (Kepler\,$\approx$\,R-band, mag). } %\label{tab:largetable}
\tablehead{\colhead{Name}  & \colhead{H$_{V}$}  & \colhead{a}  &  \colhead{e}  &  \colhead{i}  
&  \colhead{Dynamical group} & \colhead{$\langle m_{11}^R(\alpha) \rangle$} & \colhead{$\langle \alpha \rangle$} & 
\colhead{$m_{110}^R(\alpha)$} }
\label{table:orbital}
\colnumbers
\startdata
\sn & 5.68 & 37.8239563 & 0.0399826 & 4.61245 & hot classical  &    5.24   &    1.45  &   5.23$\pm$0.02 \\
\de & 4.94 & 55.5040117 & 0.4168371 & 7.62938 & 2:5 resonance  &    4.45   &    1.49  &   4.20$\pm$0.06 \\
\cm & 6.68 & 42.1255750 & 0.0640919 & 3.75516 & cold classical &    6.75   &    1.18  &   6.54$\pm$0.16 \\
\ok & 6.0 & 46.5813354 & 0.1403453 & 4.88465 & hot classical   &    6.56   &    1.35  &   6.32$\pm$0.18 \\
\hz & 6.6 & 43.0180466 & 0.0323816 & 2.93273 & cold classical  &    6.55   &    1.20  &   6.35$\pm$0.16 \\
\kn & 6.6 & 44.0637410 & 0.0956953 & 2.64496 & cold classical  &    7.08   &    1.30  &   6.85$\pm$0.17 \\
%
\qb & 6.8 & 42.7192221 & 0.0995969 & 1.79485 & cold classical  &    6.62   &    1.35  &   6.38$\pm$0.18 \\
\qj & 6.2 & 44.1753883 & 0.0365290 & 2.15477 & cold classical  &    5.82   &    1.22  &   5.61$\pm$0.16 \\
\qt & 6.2 & 37.0258514 & 0.0220311 & 1.84662 & inner classical &    7.62   &    1.47  &   7.37$\pm$0.20 \\
\qx & 6.3 & 44.2115741 & 0.0270365 & 0.90745 & cold classical  &    6.66   &    1.25  &   6.45$\pm$0.17 \\
%
\xd & 5.8 & 39.2882985 & 0.1118632 & 18.14109 & plutino        &    5.99    &   1.44  &   5.74$\pm$0.19 \\
\xp & 7.77 & 42.0465415 & 0.2142201 & 2.61611 & 3:5 resonance  &    7.51    &   1.52  &   7.25$\pm$0.20 \\
\xu & 6.68 & 43.2829795 & 0.0780917 & 6.52230 & hot classical  &    6.38    &   1.18  &   6.18$\pm$0.16 \\
%
\yh & 5.58 & 42.1828001 & 0.1369339 & 11.09996 & 3:5 resonance  &   5.75    &   1.50  &   5.49$\pm$0.20 \\
\cy & 6.16 & 53.7570643 & 0.3432009 & 15.76009 & 5:12 resonance &   7.27    &   1.50  &   7.01$\pm$0.22 \\
\gj & 5.4 & 44.5446573 & 0.1073526 & 11.57225 & hot classical   &   6.11    &   1.30  &   5.89$\pm$0.17 \\
%
\vs & 6.3 & 44.8124374 & 0.1201659 & 3.00131 & cold classical   &   6.09    &   1.31  &   5.86$\pm$0.17 \\
\vt & 5.7 & 42.2145036 & 0.0356054 & 1.16426 & cold classical   &   5.43    &   1.30  &   5.21$\pm$0.17 \\
\vu & 5.9 & 38.9541796 & 0.2103117 & 1.37856 & plutino          &   5.72    &   1.38  &   5.48$\pm$0.18 \\
%
\fc & 7.41 & 35.0390366 & 0.0839447 & 2.37160 & 4:5 resonance   &   6.92    &   1.71  &   6.62$\pm$0.23 \\
\fe & 6.37 & 48.4332947 & 0.2592514 & 3.38301 & 1:2 resonance   &   6.53    &   1.43  &   6.18$\pm$0.46 \\
\gh & 6.0 & 44.4898956 & 0.0844735 & 1.10267 & cold classical   &   6.16    &   1.40  &   6.20$\pm$0.64 \\
\qa & 6.9 & 38.2803717 & 0.0583336 & 3.42715 & inner classical  &   6.80    &   1.48  &   6.54$\pm$0.20 \\
\qw  & 5.0 & 43.6941429 & 0.0734856 & 10.36787 & hot classical  &   4.65    &   1.26  &   4.43$\pm$0.17 \\ 
\ys & 6.8 & 43.4354691 & 0.0266317 & 3.73349 & cold classical   &   6.19    &   1.05  &   6.01$\pm$0.14 \\ 
%
\tf & 6.3 & 79.8663748 & 0.5072393 & 23.23663 & scattered disk  &   6.02    &   1.37  &   5.78$\pm$0.18 \\
\tv & 6.9 & 47.3800039 & 0.2722973 & 9.78559 & 1:2 resonance    &   7.21    &   1.63  &   6.93$\pm$0.22 \\
\xr & 4.3 & 57.2561486 & 0.1073786 & 46.79343 & scattered disk  &   3.96    &   0.98  &   3.79$\pm$0.13 \\
%
\eo & 6.21 & 45.8983194 & 0.0739658 & 3.41227 & cold classical  &   6.16    &   1.23  &   5.95$\pm$0.16 \\
\ez & 7.13 & 39.6766516 & 0.1557282 & 1.77550 & plutino         &   7.21    &   1.47  &   6.95$\pm$0.19 \\
\rs & 5.18 & 47.7306105 & 0.2003342 & 10.02598 & 1:2 resonance  &   4.76    &   1.27  &   4.54$\pm$0.17 \\
\tb & 4.55 & 75.9529877 & 0.3917797 & 26.49004 & scattered disk &   4.63    &   1.17  &   4.63$\pm$0.13 \\
%
\cs & 6.27 & 42.2933803 & 0.1579361 & 15.94423 & 3:5 resonance  &   6.33    &   1.58  &   6.06$\pm$0.21 \\
\yg & 6.2 & 55.2226347 & 0.4040541 & 5.16230 & 2:5 resonance    &   5.91    &   1.53  &   5.64$\pm$0.20 \\
\ep & 5.54 & 47.8794282 & 0.3094197  & 18.86373 & 1:2 resonance &   5.55    &   1.55  &   5.29$\pm$0.20 \\
\et & 5.26 & 62.5104891 & 0.3659258 & 30.58345 & scattered disk &   4.71    &   1.44  &   4.46$\pm$0.19 \\
\fcten  & 5.88 & 39.0790779 & 0.0535418 & 39.73235 & plutino    &   4.49    &   1.45  &   4.24$\pm$0.19 \\
%
\jf & 5.43 & 41.6753240 & 0.1307786 & 27.64613 & hot classical         &  5.50  &  1.26 &  5.28$\pm$0.17 \\
\dw & 6.06 & 41.2840227 & 0.0379671 & 18.99296 & hot classical         &  6.12  &  1.28 &  5.90$\pm$0.17 \\
\apthirteen & 5.67 & 57.5543033 & 0.3668924 & 3.33318 & 3:8 resonance  &  5.41  &  1.10 &  5.22$\pm$0.15 \\
\at & 4.9 & 61.6173083 & 0.4217387 & 28.12567 & scattered disk         &. 4.82. &  0.81 &  4.68$\pm$0.11 \\
\fa & 6.2 & 44.4091197 & 0.0426125 & 1.53768 & cold classical          &  6.22  &  1.14 &  6.02$\pm$0.15 \\
\jv & 6.35 & 42.9996513 & 0.0424042 & 3.21441 & cold classical         &  6.23  &  1.29 &  6.01$\pm$0.17 \\
%
\am & 5.2 & 47.0230084 & 0.1423797 & 7.18355 & hot classical           &  5.14  &  1.06 &  4.94$\pm$0.14 \\
\df & 5.56 & 42.8307595 & 0.0456454 & 23.68086 & hot classical         &  5.58  &  1.28 &  5.36$\pm$0.17 \\
\djfourteen & 6.61 & 38.1807753 & 0.0232355 & 6.93181 & 4:13 resonance &  6.76  &  1.52 &  6.50$\pm$0.20 \\
\ezfourteen & 3.92 & 52.5242987 & 0.2263985 & 10.25719 & scattered disk&  4.09  &  0.94 &  3.93$\pm$0.12 \\
\gdfourteen & 6.71 & 90.1672371 & 0.6157590 & 4.74239 & scattered disk &  6.78  &  1.47 &  6.52$\pm$0.19 \\
\gefourteen & 6.56 & 56.0228149 & 0.4158196 & 0.80808 & 2:5 resonance  &  6.73  &  1.65 &  6.45$\pm$0.22 \\
\gjfourteen & 7.5 & 39.8224386 & 0.2801272 & 17.22611 & plutino        &  7.55  &  1.90 &  7.22$\pm$0.25 \\
\hf & 5.9 & 61.7601933 & 0.4255242 & 9.71007 & scattered disk          &  6.05  &  1.55 &  5.78$\pm$0.20 \\
\jq & 7.38 & 39.7549394 & 0.2233159 & 7.97258 & plutino                &  7.32  &  1.78 &  7.01$\pm$0.24 \\
\ls & 6.2 & 43.6029549 & 0.0681892 & 3.82390 & cold classical          &  6.17  &  1.04 &  5.99$\pm$0.14 \\
\wanine & 6.0 & 44.0261031 & 0.0531885 & 3.00216 & cold classical      &  6.13  &  1.06 &  5.95$\pm$0.14 \\
\waten & 5.9 & 45.4170544 & 0.0367855  & 2.15623 & cold classical      &  5.89  &  1.08 &  5.71$\pm$0.14 \\
\wj & 6.71 & 68.4462110 & 0.4912992 & 24.36183 & scattered disk        &  6.69  &  1.67 &  6.41$\pm$0.22 \\
\wo & 6.3 & 43.9992014  & 0.0923767  & 3.75719 & cold classical        &  6.19  &  1.28 &  5.96$\pm$0.17 \\
\ws & 5.55 & 54.9409609 & 0.3708612 & 8.90970 & 2:5 resonance          &  5.65  &  1.25 &  5.44$\pm$0.16 \\
\ye & 5.53 & 59.1067258 & 0.3757100 & 26.91854 & scattered disk        &  5.42  &  1.17 &  5.22$\pm$0.16 \\
\yj & 6.84 & 39.3040558 & 0.1951859 & 7.28212 & plutino                &  7.13  &  1.60 &  6.86$\pm$0.21 \\
%
\bbfifteen & 6.7 & 63.1405090  & 0.4398171 & 27.62710 & scattered disk &  6.59  &  1.32 &  6.37$\pm$0.17 \\
\bc & 6.7 & 55.2299967  & 0.4166677 & 1.72294 & 2:5 resonance          &  6.94  &  1.52 &  6.68$\pm$0.20 \\
\bz & 4.81 & 47.2750427 & 0.1850024 & 11.35989 & other TNO             &  5.00  &  1.03 &  4.82$\pm$0.14 \\
\da & 7.47  & 72.9126980 & 0.5110819 & 27.66698 & scattered disk       &  7.32  &  1.51 &  7.06$\pm$0.20 \\
Borasisi & 5.9 & 43.8343021 & 0.0906165 & 0.56342 & cold classical     &  5.90  &  1.08 &  5.72$\pm$0.14 \\
Praamzius & 5.75 & 42.5834453 & 0.0104114 & 1.09950 & cold classical   &  5.93  &  1.24 &  5.72$\pm$0.17 \\ \hline
\enddata
\end{deluxetable*}
%\endlongtable
\normalsize
%cubewano 4.5 inkclinacio alatt cold, felette hot

==> figures/aei_m11r.tex <==
\startlongtable
\begin{deluxetable*}{cccccc|ccc}
\tabletypesize{\scriptsize}
\tablecaption{Summary table of the main orbital characteristics and dynamical classification of our targets. 
The columns are: (1) name and/or provisional designation; (2) V-band absolute magnitude (mag); (3) semi-major axis (au);
(4) eccentricity; (5) inclination (deg); (6) dynamical class or mean-motion resonance with Neptune. 
Cold and hot classicals are separated by the inclination i\,=\,4\fdg5 \citep[see e.g.][]{Gladman2008; 
(7) phase-angle-uncorrected mean absolute brightness (Kepler\,$\approx$\,R-band, mag); (8) mean phase angle (deg);
(9) phase-angle-corrected mean absolute brightness (Kepler\,$\approx$\,R-band, mag). } %\label{tab:largetable}
\tablehead{\colhead{Name}  & \colhead{H$_{V}$}  & \colhead{a}  &  \colhead{e}  &  \colhead{i}  
&  \colhead{Dynamical group} & \colhead{$\langle m_{11}^R(\alpha) \rangle$} & \colhead{$\langle \alpha \rangle$} & \colhead{} 
}
\colnumbers
\startdata
\sn & 5.68 & 37.8239563 & 0.0399826 & 4.61245 & hot classical  &    5.24   &    1.45  &   5.09$\pm$0.11 \\
\de & 4.94 & 55.5040117 & 0.4168371 & 7.62938 & 2:5 resonance  &    4.45   &    1.49  &   4.30$\pm$0.11 \\
\cm & 6.68 & 42.1255750 & 0.0640919 & 3.75516 & cold classical &    6.75   &    1.18  &   6.62$\pm$0.09 \\
\ok & 6.0 & 46.5813354 & 0.1403453 & 4.88465 & hot classical   &    6.56   &    1.35  &   6.42$\pm$0.10 \\
\hz & 6.6 & 43.0180466 & 0.0323816 & 2.93273 & cold classical  &    6.55   &    1.20  &   6.43$\pm$0.09 \\
\kn & 6.6 & 44.0637410 & 0.0956953 & 2.64496 & cold classical  &    7.08   &    1.30  &   6.94$\pm$0.10 \\

\qb & 6.8 & 42.7192221 & 0.0995969 & 1.79485 & cold classical  &    6.62   &    1.35  &   6.48$\pm$0.10 \\
\qj & 6.2 & 44.1753883 & 0.0365290 & 2.15477 & cold classical  &    5.82   &    1.22  &   5.69$\pm$0.09 \\
\qt & 6.2 & 37.0258514 & 0.0220311 & 1.84662 & inner classical &    7.62   &    1.47  &   7.47$\pm$0.11 \\
\qx & 6.3 & 44.2115741 & 0.0270365 & 0.90745 & cold classical  &    6.66   &    1.25  &   6.53$\pm$0.10 \\
%
\xd & 5.8 & 39.2882985 & 0.1118632 & 18.14109 & plutino        &    5.99    &   1.44  &   5.84$\pm$0.11 \\
\xp & 7.77 & 42.0465415 & 0.2142201 & 2.61611 & 3:5 resonance  &    7.51    &   1.52  &   7.36$\pm$0.11 \\
\xu & 6.68 & 43.2829795 & 0.0780917 & 6.52230 & hot classical  &    6.38    &   1.18  &   6.26$\pm$0.09 \\
%
\yh & 5.58 & 42.1828001 & 0.1369339 & 11.09996 & 3:5 resonance  &   5.75    &   1.50  &   5.59$\pm$0.11 \\
\cy & 6.16 & 53.7570643 & 0.3432009 & 15.76009 & 5:12 resonance &   7.27    &   1.50  &   7.12$\pm$0.14 \\
\gj & 5.4 & 44.5446573 & 0.1073526 & 11.57225 & hot classical   &   6.11    &   1.30  &   5.98$\pm$0.10 \\
%
\vs & 6.3 & 44.8124374 & 0.1201659 & 3.00131 & cold classical   &   6.09    &   1.31  &   5.95$\pm$0.10 \\
\vt & 5.7 & 42.2145036 & 0.0356054 & 1.16426 & cold classical   &   5.43    &   1.30  &   5.30$\pm$0.10 \\
\vu & 5.9 & 38.9541796 & 0.2103117 & 1.37856 & plutino          &   5.72    &   1.38  &   5.57$\pm$0.10 \\
%
\fc & 7.41 & 35.0390366 & 0.0839447 & 2.37160 & 4:5 resonance   &   6.92    &   1.71  &   6.74$\pm$0.13 \\
\fe & 6.37 & 48.4332947 & 0.2592514 & 3.38301 & 1:2 resonance   &   6.53    &   1.43  &   6.38$\pm$0.11 \\
\gh & 6.0 & 44.4898956 & 0.0844735 & 1.10267 & cold classical   &   6.16    &   1.40  &   6.01$\pm$0.10 \\
\qa & 6.9 & 38.2803717 & 0.0583336 & 3.42715 & inner classical  &   6.80    &   1.48  &   6.64$\pm$0.11 \\
\qw  & 5.0 & 43.6941429 & 0.0734856 & 10.36787 & hot classical  &   4.65    &   1.26  &   4.52$\pm$0.09 \\ 
\ys & 6.8 & 43.4354691 & 0.0266317 & 3.73349 & cold classical   &   6.19    &   1.05  &   6.09$\pm$0.08 \\ 
%
\tf & 6.3 & 79.8663748 & 0.5072393 & 23.23663 & scattered disk  &   6.02    &   1.37  &   5.87$\pm$0.10 \\
\tv & 6.9 & 47.3800039 & 0.2722973 & 9.78559 & 1:2 resonance    &   7.21    &   1.63  &   7.04$\pm$0.12 \\
\xr & 4.3 & 57.2561486 & 0.1073786 & 46.79343 & scattered disk  &   3.96    &   0.98  &   3.85$\pm$0.07 \\
%
\eo & 6.21 & 45.8983194 & 0.0739658 & 3.41227 & cold classical  &   6.16    &   1.23  &   6.03$\pm$0.09 \\
\ez & 7.13 & 39.6766516 & 0.1557282 & 1.77550 & plutino         &   7.21    &   1.47  &   7.05$\pm$0.11 \\
\tb & 4.55 & 75.9529877 & 0.3917797 & 26.49004 & scattered disk &   4.63    &   1.17  &   4.51$\pm$0.09 \\
\rs & 5.18 & 47.7306105 & 0.2003342 & 10.02598 & 1:2 resonance  &   4.76    &   1.27  &   4.62$\pm$0.09 \\
%
\cs & 6.27 & 42.2933803 & 0.1579361 & 15.94423 & 3:5 resonance  &   6.33    &   1.58  &   6.17$\pm$0.12 \\
\yg & 6.2 & 55.2226347 & 0.4040541 & 5.16230 & 2:5 resonance    &   5.91    &   1.53  &   5.75$\pm$0.11 \\
\ep & 5.54 & 47.8794282 & 0.3094197  & 18.86373 & 1:2 resonance &   5.55    &   1.55  &   5.39$\pm$0.11 \\
\et & 5.26 & 62.5104891 & 0.3659258 & 30.58345 & scattered disk &   4.71    &   1.44  &   4.56$\pm$0.11 \\
\fcten  & 5.88 & 39.0790779 & 0.0535418 & 39.73235 & plutino    &   4.49    &   1.45  &   4.33$\pm$0.11 \\
%
\jf & 5.43 & 41.6753240 & 0.1307786 & 27.64613 & hot classical         &  5.50  &  1.26 &  5.36$\pm$0.09 \\
\dw & 6.06 & 41.2840227 & 0.0379671 & 18.99296 & hot classical         &  6.12  &  1.28 &  5.99$\pm$0.10 \\
\apthirteen & 5.67 & 57.5543033 & 0.3668924 & 3.33318 & 3:8 resonance  &  5.41  &  1.10 &  4.73$\pm$0.06 \\
\fa & 6.2 & 44.4091197 & 0.0426125 & 1.53768 & cold classical          &  6.22  &  1.14 &  6.10$\pm$0.09 \\
\jv & 6.35 & 42.9996513 & 0.0424042 & 3.21441 & cold classical         &  6.23  &  1.29 &  6.09$\pm$0.10 \\
%
\am & 5.2 & 47.0230084 & 0.1423797 & 7.18355 & hot classical           &  5.14  &  1.06 &  5.03$\pm$0.08 \\
\df & 5.56 & 42.8307595 & 0.0456454 & 23.68086 & hot classical         &  5.58  &  1.28 &  5.45$\pm$0.09 \\
\djfourteen & 6.61 & 38.1807753 & 0.0232355 & 6.93181 & 4:13 resonance &  6.76  &  1.52 &  6.60$\pm$0.11 \\
\ezfourteen & 3.92 & 52.5242987 & 0.2263985 & 10.25719 & scattered disk&  4.09  &  0.94 &  3.99$\pm$0.07 \\
\gdfourteen & 6.71 & 90.1672371 & 0.6157590 & 4.74239 & scattered disk &  6.78  &  1.47 &  6.62$\pm$0.11 \\
\gefourteen & 6.56 & 56.0228149 & 0.4158196 & 0.80808 & 2:5 resonance  &  6.73  &  1.65 &  6.56$\pm$0.12 \\
\gjfourteen & 7.5 & 39.8224386 & 0.2801272 & 17.22611 & plutino        &  7.55  &  1.90 &  7.35$\pm$0.14 \\
\hf & 5.9 & 61.7601933 & 0.4255242 & 9.71007 & scattered disk          &  6.05  &  1.55 &  5.89$\pm$0.12 \\
\jq & 7.38 & 39.7549394 & 0.2233159 & 7.97258 & plutino                &  7.32  &  1.78 &  7.13$\pm$0.13 \\
\ls & 6.2 & 43.6029549 & 0.0681892 & 3.82390 & cold classical          &  6.17  &  1.04 &  6.06$\pm$0.08 \\
\wanine & 6.0 & 44.0261031 & 0.0531885 & 3.00216 & cold classical      &  6.13  &  1.06 &  6.02$\pm$0.08 \\
\waten & 5.9 & 45.4170544 & 0.0367855  & 2.15623 & cold classical      &  5.89  &  1.08 &  5.78$\pm$0.08 \\
\wj & 6.71 & 68.4462110 & 0.4912992 & 24.36183 & scattered disk        &  6.69  &  1.67 &  6.52$\pm$0.12 \\
\wo & 6.3 & 43.9992014  & 0.0923767  & 3.75719 & cold classical        &  6.19  &  1.28 &  6.05$\pm$0.10 \\
\ws & 5.55 & 54.9409609 & 0.3708612 & 8.90970 & 2:5 resonance          &  5.65  &  1.25 &  5.52$\pm$0.09 \\
\ye & 5.53 & 59.1067258 & 0.3757100 & 26.91854 & scattered disk        &  5.42  &  1.17 &  5.30$\pm$0.09 \\
\yj & 6.84 & 39.3040558 & 0.1951859 & 7.28212 & plutino                &  7.13  &  1.60 &  6.97$\pm$0.12 \\
%
\bbfifteen & 6.7 & 63.1405090  & 0.4398171 & 27.62710 & scattered disk &  6.59  &  1.32 &  6.46$\pm$0.10 \\
\bc & 6.7 & 55.2299967  & 0.4166677 & 1.72294 & 2:5 resonance          &  6.94  &  1.52 &  6.78$\pm$0.11 \\
\bz & 4.81 & 47.2750427 & 0.1850024 & 11.35989 & other TNO             &  5.00  &  1.03 &  4.89$\pm$0.08 \\
\da & 7.47  & 72.9126980 & 0.5110819 & 27.66698 & scattered disk       &  7.32  &  1.51 &  7.16$\pm$0.11 \\
Borasisi & 5.9 & 43.8343021 & 0.0906165 & 0.56342 & cold classical     &  5.90  &  1.08 &  5.79$\pm$0.08 \\
Praamzius & 5.75 & 42.5834453 & 0.0104114 & 1.09950 & cold classical   &  5.93  &  1.24 &  5.80$\pm$0.10 \\ \hline
\enddata
\end{deluxetable*}
%\endlongtable
\normalsize

%cubewano 4.5 inkclinacio alatt cold, felette hot

==> figures/individual6.tex <==

\onecolumngrid
%%% 2003 GH55
\paragraph{\gh}
The main frequency/period we identified is f\,=\,0.114\,$\pm$0.002\,h, P\,=\,210.526$\pm$3.693\,h, with a light curve amplitude of $\Delta m$\,=\,0.402$\pm$0.060. A secondary, tentative frequency was also found (S/N\,=\,2.74\,$\sigma$ in the Fourier spectrum), with f\,=\,2.5618$\pm$0.0029\,c/d, P\,=\,9.3683$\pm$0.01062\,h and $\Delta m$\,=\,0.165$\pm$0.034. %The significance of the secondary frequency is notably lower than that of the primary. 

%%% 2014 JQ80
\paragraph{\jq} A prominent contant binary was detected for \jq by \citet{TS18} (TS18), with a double peak light curve period of P\,=\,12.16\,h. Our analysis provided the period P\,=\,6.079\,h, (f\,=\,3.948 c/d) with the highest signal-to-noise over the r.m.s. noise in the residual spectrum. This is exactly the half-period of that found by TS18, and their single-peak period. While the associated light curve amplitude is definitely smaller than the TS18 one, this is expected considering the faintness of the target and the relative accuracy that could be achieved in K2 measurements due to the small telescope size. Finding the previously identified period of \jq\, is a good example that our method can effectively select the 'right' periods from multiple possibilities. 

%%% 2015 BB519
\paragraph{\bbfifteen}
A single frequency was identified at f\,=\,0.328$\pm$0.002\,c/d, P\,=\,73.171$\pm$0.446\,h and  $\Delta$m\,=\,0.560$\pm$0.091. 

%%% 2015 BC519
\paragraph{\bc}
A single, tentative frequency was identified at f\,=\,2.688$\pm$0.007\,c/d, P\,=\,8.929$\pm$0.023\,h and  $\Delta$m\,=\,0.5139$\pm$0.095. Other peaks at lower frequencies are not considered as viable due to the increased noise in this part of the spectrum. 


\paragraph{\bz}%2015bz518}
Two prominent peaks were identified: one at f\,=\,0.760$\pm$0.004\,c/d, P\,=\,31.578$\pm$0.083\,h, $\Delta$m\,=\,0.392$\pm$0.079, and another one at f\,=\,1.476$\pm$0.004\,c/d, P\,=\,16.260$\pm$0.022\,h, $\Delta$m\,=\,0.373$\pm$0.076. The first one is very close to the double period of the second one, but the light curve folded with the originally identified P\,=\,31.578$\pm$0.083\,h period shows a behaviour rather different from that folded with the double period of the other frequency, P\,=\,32.520\,h (see Fig.~\ref{fig:2015bz518} below). Due to its higher significance we use P\,=\,31.578$\pm$0.083\,h as primary period. 

%%% 2015 DA225
\paragraph{\da}%2015225}
We found a light curve frequency of f\,=\,6.7961$\pm$0.0034\,c/d, P\,=\,3.531$\pm$0.002\,h, with $\Delta m$\,=\,0.511$\pm$0.128. Another minimum was identified in the phase dispersion at f\,=\,0.668$\pm$0.004\,c/d, P\,=\,35.928$\pm$0.188\,h, with $\Delta m$\,=\,0.484$\pm$0.119. Due to the higher significance of the higher frequency (shorter period) over the noise obtained both in the Fourier and the in the periodogram analysis we consider that (f\,=\,6.7961$\pm$0.0034\,c/d) as the primary period. 

\paragraph{Borasisi}
\citet{Kern2006} obtained a rotation period of P\,=\,6.4$\pm$0.1\,h, using data from one single night to determine the light curve period, and another night with some spare phase coverage almost a year later, when the fixed period from the first date was used to phase the data.  We could not recover this period from our data, but identified a single prominent period at f\,=\,1.208$\pm$0.002\,c/d or P\,=\,19.868\,$\pm$0.032\,h, with an amplitude of $\Delta m$\,=\,0.216$\pm$0.057. 

\paragraph{Praamzius}
A prominent minimum was identified at the low-frequency part of the spectum at f\,=\,0.352$\pm$0.004\,c/d, P\,=\,68.182$\pm$0.775\,h, with a large light curve ampltiude of $\Delta m$\,=\,1.433$\pm$0.181. 
There is another, prominent minimum at the high-frequency part at f\,=\,9.108$\pm$0.002\,c/d (P\,=2.635$\pm$0.001\,h, $\Delta m$\,=\,0.536$\pm$0.218) that technically meets the criteria of a detection. However, we consider this frequency as tentative and use f\,=\,0.352$\pm$0.004\,c/d as primary frequency. 


%%%%%%%%%% Big figure 0 %%%%%%%%%%%%%%%%%%%%%
%\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}

%%%%%%%
\begin{figure*}[ht!]
%\centering
\hbox{%\centering
\includegraphics[width=0.25\textwidth]{{figures/Borasisi_full_lc_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/borasisi_fp}.pdf}
\includegraphics[width=0.25\textwidth]{{figures/Borasisi_P=19.868h_BW}.jpg}
}
%\noindent\rule{1.03\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/Praamzius_full_lc_BW.jpg}
\includegraphics[width=0.25\textwidth]{figures/praamzius_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/Praamzius_P=68.182h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/Praamzius_P=2.635h_BW}.jpg}
}
%\noindent\rule{1.03\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/1998SN165_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/1998sn165_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/1998SN165_P=5.646h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/1998SN165_P=2.817h_BW}.jpg}
}
%\noindent\rule{1.03\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/1999DE9_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/1999de9_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/1999DE9_P=22.947h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/1999DE9_P=12.745h_BW}.jpg}
}
%\noindent\rule{1.03\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2000OK67_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2000ok67_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2000OK67_P=33.803h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2001HZ58_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2001hz58_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2001HZ58_P=5.138h_BW}.jpg}
}
\caption{For each target (one target a row) we present the following figures, from left to right: 1) Unfolded light curve; 
2) Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.; 3-(4) Light curves folded by the periods/frequencies identified. Here we present the figures for Borasisi, Praamzius, \sn, \de, \ok\, and \hz. \label{fig:big0}}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%% 1
\begin{figure*}[ht!]
%\centering
%\noindent\rule{\textwidth}{1pt}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2001XP254_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2001XP254_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2001XP254_P=46.720h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2001XU254_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2001XU254_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2001XU254_P=17.647h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2001XU254_P=35.294h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2001YH140_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2001yh140_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2001YH140_P=27.397h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2001YH140_P=13.706h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2002VS130_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2002vs130_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2002VS130_P=8.639h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2003FC128_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2003fc128_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2003FC128_P=27.675h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2003FE128_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2003fe128_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2003FE128_P=7.727h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2003FE128_P=41.237h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2003GH55_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2003gh55_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2003GH55_P=210.526h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2003GH55_P=9.368h_BW}.jpg}
}
\caption{The same as Fig.~\ref{fig:big0}, but for \xp, \xu, \yh, \vs, \fc, \fe, and \gh.  \label{fig:big1}}
\end{figure*}

%%%%%%% 2 
\begin{figure*}[ht!]
%\centering
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2003QW90_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2003qw90_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2003QW90_P=86.331h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2003QW90_P=44.444h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2003YS179_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2003ys179_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2003YS179_P=19.293h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2005EO304_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2005EO304_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2005EO304_P=36.474h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2005EZ296_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2005EZ296_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2005EZ296_P=4.730h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2005EZ296_P=40.268h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2009YG19_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2009yg19_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2009YG19_P=3.793h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2009YG19_P=7.581h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2010EP65_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2010ep65_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2010EP65_P=12.422h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2010ET65_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2010ET65_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2010ET65_P=16.529h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2010ET65_P=33.149h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\caption{The same as Fig.~\ref{fig:big0}, but for \qw, \ys, \eo, \ez, \yg, \ep and \et. }
\label{fig:big2}
\end{figure*}
%%%%

%%%%% Big figure 3 %%%%%%%
\begin{figure*}[ht!]
%\centering
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2011JF31_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2011jf31_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2011JF31_P=2.658h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2011JF31_P=5.316h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2012DW98_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2012dw98_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2012DW98_P=30.380h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2013AP183_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2013ap183_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2013AP183_P=5.008h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2013AT183_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2013aT183_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2013AT183_P=78.788h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2013JV65_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2013jv65_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2013JV65_P=6.027h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014EZ51_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014ez51_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014EZ51_P=3.200h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014GD54_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014gd54_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014GD54_P=44.280h_BW}.jpg}
}
\caption{The same as Fig.~\ref{fig:big0}, but for \jf, \dw, \apthirteen, \at, \jv, \ezfourteen, and \gdfourteen.}
\label{fig:big3}
\end{figure*}
%%%%

%%%%%%% Big figure 4 %%%%%%%%
\begin{figure*}[ht!]
%\centering
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014HF200_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014hf200_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014HF200_P=4.992h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014JQ80_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014jq80_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014JQ80_P=6.079h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2014JQ80_P=12.158h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014WJ510_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014wj510_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014WJ510_P=40.541h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014WS510_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014ws510_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014WS510_P=25.009h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2014YE50_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2014ye50_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2014YE50_P=56.970h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2015BB519_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2015bb519_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2015BB519_P=73.202h_BW}.jpg}
}
%\noindent\rule{\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2015BC519_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2015bc519_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2015BC519_P=8.899h_BW}.jpg}
}
\caption{The same as Fig.~\ref{fig:big0} but for \hf, \jq, \wj, \ws, \ye, \bbfifteen\, and \bc.}
\label{fig:big4}
\end{figure*}
%%%%


%%%%%%% Big figure 5 %%%%%%%%
\begin{figure}[ht!]
%\centering
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2015BZ518_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2015bz518_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2015BZ518_P=16.260h_BW}.jpg}
%\includegraphics[width=0.25\textwidth]{{figures/2015BZ518_P=32.520h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2015BZ518_P=31.579h_BW}.jpg}
}
%\noindent\rule{1.03\textwidth}{1pt}
\hbox{
\includegraphics[width=0.25\textwidth]{figures/2015DA225_full_lc_BW.pdf}
\includegraphics[width=0.25\textwidth]{figures/2015da225_fp.pdf}
\includegraphics[width=0.25\textwidth]{{figures/2015DA225_P=3.531h_BW}.jpg}
\includegraphics[width=0.25\textwidth]{{figures/2015DA225_P=35.928h_BW}.jpg}
}
\caption{The same as Fig.~\ref{fig:big0} but for \bz\, and \da.}
\label{fig:big5}
\end{figure}
%%%%




==> freq_table.tex <==
%\begin{tabular}{lccccccc}
%Target & \multicolumn{2}{c}{frequency} & \multicolumn{2}{c}{Period} & \multicolumn{2}{c}{Amplitude} & flag\\ 
1998sn165 & & & &        \\ 
1999de9 &       \\
2000cm105 &       \\
2000ok67 &       \\
2001hz58 &       \\
2001kn76 &       \\
2001qb298 &       \\
2001qj298 &       \\
2001qt322 &       \\
2001qx297 &       \\
2001xd255 &       \\
2001xp254 &       \\
2001xu254 &       \\
2001yh140 &       \\
2001yh140.lc &       \\
2002cy224 &       \\
2002gj32 &       \\
2002gv31 &       \\
2002vs130 &       \\
2002vt130 &       \\
2002vu130 &       \\
2003fc128 &       \\
2003fe128 &       \\ \hline
2003gh55 &  0.114 & 0.002 & 210.526 & 3.693 & 0.402 & 0.060 & p & \\
         &  2.561 & 0.003 & 9.3683 & 0.01062 & 0.165 & 0.034 & s/t & \\ \hline
2003qa92.1 &       \\
2003qa92.2 &       \\
2003qa92 &       \\
2003qw90 &       \\
2003ys179 &       \\
2004tf282 &       \\
2004tv357 &       \\
2004xr190 &       \\
2005eo304 &       \\
2005ez296 &       \\
2005rs43 &       \\
2005tb190 &       \\
2007jj43 &       \\
2007or10 &       \\
2008cs190 &       \\
2009yg19 &       \\
2010ep65 &       \\
2010et65 &       \\
2010fc49 &       \\
2011jf31 &       \\
2012dw98 &       \\
2013ap183 &       \\
2013at183 &       \\
2013fa28 &       \\
2013jv65 &       \\
2014am55 &       \\
2014df143 &       \\
2014dj143 &       \\
2014ez51 &       \\
2014gd54 &       \\
2014ge45 &       \\
2014gj54 &       \\
2014hf200 &       \\
2014jq80 &       \\
2014ls28 &       \\
2014wa509 &       \\
2014wa510 &       \\
2014wj510 &       \\
2014wo509 &       \\
2014ws510 &       \\
2014ye50 &       \\
2014yj50 &       \\
2015bb519 &       \\
2015bc519 &  2.688 & 0.007 & 8.928 & 0.023 & 0.514 & 0.095 & p/t &    \\ \hline
2015bz518 &  0.760 & 0.004 & 31.578 & 0.083 & 0.392 & 0.079 & p &     \\ 
          &  1.476 & 0.004 & 16.260 & 0.022 & 0.373 & 0.076 & s & \\ \hline
\da &   6.7961 & 0.0034 & 3.531 & 0.002 &  0.511 & 0.128 & p \\
          &   0.668 & 0.004 & 35.928 & 0.188 & 0.484 & 0.119 & s/t \\ \hline
Borasisi & 1.208 &  0.002 & 19.868 & 0.032 & 0.216 & 0.057 & p & 6.4$\pm$0.1 & K06 \\ \hline
Praamzius & 0.352 & 0.004 & 68.182 & 0.775 & 1.433 & 0.181 & p & &  \\
          & 9.108 & 0.002 & 2.635 & 0.001 & 0.536 & 0.218 & s/t & & \\
%quaoar &       \\
%\end{tabular}

%We found a light curve frequency of f\,=\,6.7961$\pm$0.0034\,c/d, P\,=\,3.531$\pm$0.002\,h, with $\Delta m$\,=\,0.511$\pm$0.128. Another minimum was identified in the phase dispersion at f\,=\,0.668$\pm$0.004\,c/d, P\,=\,35.928$\pm$0.188\,h, with $\Delta m$\,=\,0.484$\pm$0.119. Due to the higher significance of the higher frequency (shorter period) over the noise obtained both in the Fourier and the in the periodogram analysis we consider that (f\,=\,6.7961$\pm$0.0034\,c/d) as the primary period. 

==> individual.tex <==
\subsection*{1998sn165}
\subsection*{1999de9}
\subsection*{2000cm105}
\subsection*{2000ok67}
\subsection*{2001hz58}
\subsection*{2001kn76}
\subsection*{2001qb298}
\subsection*{2001qj298}
\subsection*{2001qt322}
\subsection*{2001qx297}
\subsection*{2001xd255}
\subsection*{2001xp254}
\subsection*{2001xu254}

\subsection*{2001yh140}


\subsection*{2002cy224}
\subsection*{2002gj32}
\subsection*{2002gv31}
\subsection*{2002vs130}
\subsection*{2002vt130}
\subsection*{2002vu130}
\subsection*{2003fc128}
\subsection*{2003fe128}

\clearpage
%%%%%%%%%% 2003 GH55 %%%%%%%%%%%%%%%%%%%%%
%\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}
\subsection{2003gh55}
The main frequency/period we identified is f\,=\,0.114\,$\pm$0.002\,h, P\,=\,210.526$\pm$3.693\,h, with a light curve amplitude of $\Delta m$\,=\,0.402$\pm$0.060. A secondary, tentative frequency was also found (S/N\,=\,2.74\,$\sigma$ in the Fourier spectrum), with f\,=\,2.5618$\pm$0.0029\,c/d, P\,=\,9.3683$\pm$0.01062\,h and $\Delta m$\,=\,0.165$\pm$0.034. %The significance of the secondary frequency is notably lower than that of the primary. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{2003GH55_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{2003gh55_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{2003GH55_P=210.526h_BW.pdf}
\includegraphics[width=0.5\textwidth]{2003GH55_P=9.368h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \gh. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom row}: Light curves folded by the periods/frequencies identified.    }
\label{fig:gh55}
\end{figure*}
%%
%%
%\begin{figure*}[ht!]
%    \centering
%    
%    \caption{Light curve folded with a tentative, secondary frequency.}
%    \label{fig:freq_gh55sec}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{2003qa92}
\subsection*{2003qw90}
\subsection*{2003ys179}
\subsection*{2004tf282}
\subsection*{2004tv357}
\subsection*{2004xr190}
\subsection*{2005eo304}
\subsection*{2005ez296}
\subsection*{2005rs43}
\subsection*{2005tb190}
\subsection*{2007jj43}
\subsection*{2007or10}
\subsection*{2008cs190}
\subsection*{2009yg19}
\subsection*{2010ep65}
\subsection*{2010et65}
\subsection*{2010fc49}
\subsection*{2011jf31}
\subsection*{2012dw98}
\subsection*{2013ap183}
\subsection*{2013at183}
\subsection*{2013fa28}
\subsection*{2013jv65}
\subsection*{2014am55}
\subsection*{2014df143}
\subsection*{2014dj143}
\subsection*{2014ez51}
\subsection*{2014gd54}
\subsection*{2014ge45}
\subsection*{2014gj54}
\subsection*{2014hf200}
\subsection*{2014jq80}

\subsection*{2014wa509}
\subsection*{2014wa510}
\subsection*{2014wj510}
\subsection*{2014wo509}
\subsection*{2014ws510}
\subsection*{2014ye50}
\subsection*{2014yj50}

%%%%%%%%
\clearpage
\subsection*{2015bb519}

A single frequency was identified at f\,=\,0.328$\pm$0.002\,c/d, P\,=\,73.171$\pm$0.446\,h and  $\Delta$m\,=\,0.560$\pm$0.091. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BB519_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015bb519_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BB519_P=73.171h_BW.pdf}
%\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=32.520h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \bb. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom rows}: Light curves folded by the periods/frequencies identified (see the text for details).   \label{fig:2015bc519} }
\end{figure*}

%%%%%%%%%%%%%%
\clearpage
\subsection*{2015bc519}

A single, tentative frequency was identified at f\,=\,2.688$\pm$0.007\,c/d, P\,=\,8.929$\pm$0.023\,h and  $\Delta$m\,=\,0.5139$\pm$0.095. Other peaks at lower frequencies are not considered as viable due to the increased noise in this part of the spectrum. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BC519_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015bc519_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BC519_P=8.929h_BW.pdf}
%\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=32.520h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \gh. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom rows}: Light curves folded by the periods/frequencies identified (see the text for details).   \label{fig:2015bc519} }
\end{figure*}
%%%%%%%%%%%%%%%

\clearpage
\subsection*{\bz}%2015bz518}

Two prominent peaks were identified: one at f\,=\,0.760$\pm$0.004\,c/d, P\,=\,31.578$\pm$0.083\,h, $\Delta$m\,=\,0.392$\pm$0.079, and another one at f\,=\,1.476$\pm$0.004\,c/d, P\,=\,16.260$\pm$0.022\,h, $\Delta$m\,=\,0.373$\pm$0.076. The first one is very close to the double period of the second one, but the light curve folded with the originally identified P\,=\,31.578$\pm$0.083\,h period shows a behaviour rather different from that folded with the double period of the other frequency, P\,=\,32.520\,h (see Fig.~\ref{fig:2015bz518} below). Due to its higher significance we use P\,=\,31.578$\pm$0.083\,h as primary period. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BZ518_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015bz518_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=16.260h_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=32.520h_BW.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=31.579h_BW.pdf}
%\includegraphics[width=0.5\textwidth]{figures/2015BZ518_P=32.520h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \gh. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom rows}: Light curves folded by the periods/frequencies identified (see the text for details).   \label{fig:2015bz518} }
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage 
\subsection*{\da}%2015225}

We found a light curve frequency of f\,=\,6.7961$\pm$0.0034\,c/d, P\,=\,3.531$\pm$0.002\,h, with $\Delta m$\,=\,0.511$\pm$0.128. Another minimum was identified in the phase dispersion at f\,=\,0.668$\pm$0.004\,c/d, P\,=\,35.928$\pm$0.188\,h, with $\Delta m$\,=\,0.484$\pm$0.119. Due to the higher significance of the higher frequency (shorter period) over the noise obtained both in the Fourier and the in the periodogram analysis we consider that (f\,=\,6.7961$\pm$0.0034\,c/d) as the primary period. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015DA225_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015da225_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2015DA225_P=3.531h_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2015DA225_P=35.928h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \gh. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom row}: Light curves folded by the periods/frequencies identified.   \label{fig:borasisi} }
\end{figure*}


%%%%%%%%%%%%%%%% Borasisi %%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Borasisi}

\citet{Kern2006} obtained a rotation period of P\,=\,6.4$\pm$0.1\,h, using data from one single night to determine the light curve period, and another night with some spare phase coverage almost a year later, when the fixed period from the first date was used to phase the data.  We could not recover this period from our data, but identified a single prominent period at f\,=\,1.208$\pm$0.002\,c/d or P\,=\,19.868\,$\pm$0.032\,h, with an amplitude of $\Delta m$\,=\,0.216$\pm$0.057. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/Borasisi_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/borasisi_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/Borasisi_P=19.868h_BW.pdf}
%\includegraphics[width=0.5\textwidth]{2003GH55_P=9.368h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of \gh. 
{\sc Top-Right:} Phase dispersion versus frequency. Red arrows mark the light curve frequencies detected by our analysis.  {\sc Bottom row}: Light curves folded by the periods/frequencies identified.   \label{fig:borasisi} }
\end{figure*}

\clearpage
\subsection*{praamzius}

A prominent minimum was identified at the low-frequency part of the spectum at f\,=\,0.352$\pm$0.004\,c/d, P\,=\,68.182$\pm$0.775\,h, with a large light curve ampltiude of $\Delta m$\,=\,1.433$\pm$0.181. 
There is another, prominent minimum at the high-frequency part at f\,=\,9.108$\pm$0.002\,c/d (P\,=2.635$\pm$0.001\,h, $\Delta m$\,=\,0.536$\pm$0.218) that technically meets the criteria of a detection. However, we consider this frequency as tentative and use f\,=\,0.352$\pm$0.004\,c/d as primary frequency. 

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/Praamzius_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/praamzius_fp.pdf}}
\hbox{
\includegraphics[width=0.5\textwidth]{figures/Praamzius_P=68.182h_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/Praamzius_P=2.635h_BW.pdf}
}
\caption{{\sc Top-Left}: Unfolded light curve of Praamzius. 
{\sc Top-Right:} Phase dispersion versus frequency. The red arrows mark the light curve frequencies identified by our analysis.  {\sc Bottom row}: Light curve folded by the periods/frequencies identified.   \label{fig:praamzius} }
\end{figure*}

%\subsection*{praamzius.lc}
%\subsection*{quaoar}


==> nodetect.tex <==

\begin{figure*}[ht!]
\centering
\hbox{
\includegraphics[width=0.5\textwidth]{figures/2014LS28_full_lc_BW.pdf}
\includegraphics[width=0.5\textwidth]{figures/2014ls28.f04.pdf}}
%\hbox{
%\includegraphics[width=0.5\textwidth]{figures/Praamzius_P=68.182h_BW.pdf}
%\includegraphics[width=0.5\textwidth]{figures/Praamzius_P=2.635h_BW.pdf}
%}
\caption{{\sc Left}: Unfolded, full light curve of targets without detected light curve periods. 
{\sc Right:} Fourier spectrum of the light curve. The blue curve represents the 1$\sigma$ r.m.s. of the spectrum. The name of the target is indicated at the bottom-right corner.    \label{fig:nodetect} }
\end{figure*}

==> nonsinedetct.tex <==
\section{On the detectability of non-sinusoidal light curves}

In addition to a sinusoidal variation, we also assumed two kind of light curves, typically considered for asteroids and trans-Neptunian objects: a rotating tri-axial ellipsoid with axes $a$\,$\geq$\,$b$\,$geq$\,$c$, rotating around axis $c$, and a contact binary, with two spherical bodies or radius $r_1$\,$\geq$\,$r_2$. 
The light curve of the tri-axial ellipsoid  is obtained as:
\begin{equation}
    m(b/a,\theta) = 2.5 \log_{10} \Big[ \Big( 1 + \Big(\Big( {b\over a}\Big)^2 -1\Big) \cos^2\theta \Big)^{1\over 2} \Big]
\end{equation}
, where $\theta$ is the rotational phase angle, and we assumed equator-on viewing geometry and zero phase angle.
For the contact binary the light curve is obtained as:
%%%%
\begin{eqnarray}
    m(r_1,r_2,\theta,\phi) = 2.5 \log_{10} \Big[ 
    \frac{r_1^2}{\pi} \Big( \pi - \eta_1 + \sin \eta_1 \cos \eta_1 \Big) 
    +  \frac{r_2^2}{\pi} \Big( \pi - \eta_2 + \sin \eta_2 \cos \eta_2 \Big) 
    \Big] & ~~~\mathrm{if}~ \cos \eta_2 \geq -1 \\
    1 & \mathrm{otherwise} 
\end{eqnarray}
%%%%
where the $\eta_1$ and $\eta_2$ angles are defined as
\begin{eqnarray}
    \cos \eta_1 = (d^2 + r_1^2 - r_2^2)/(2 d r_1)  & ~~ \mathrm{and} ~~ &
    \cos \eta_2 = (d^2 + r_2^2 - r_1^2)/(2 d r_2) 
\end{eqnarray}
and $d$ is the projected separation of the two bodies:
\begin{equation}
    d = (r_1 + r_2) (\cos^2 \theta + \sin^2 \theta \cos^2 \phi)
\end{equation}
and $\theta$ and $\phi$ are the rotational phase angle and the spin axis aspect angle, respectively. 

As described in Sect.~\ref{sect:obs} we used two methods to obtain the most prominent light curve freqeuncies: the perioodogram method using .... but we also used Fourier spectrum of the light curve, obtained by {\sc Period04}. The Fourier method is expected to be less sensivitve to non-sinusoidal light curves as in these cases the spectral power, or equivalently the light curve amplitude is distributed over several peak frequencies, most prominently the overtones of the primary frequency. 

